AutoCRAT: Automatic Cumulative Reconstruction of Alert Trees

When a network is attacked, cyber defenders need to precisely identify which systems (i.e., computers or devices) were compromised and what damage may have been inflicted. This process is sometimes referred to as cyber triage and is an important part of the incident response procedure. Cyber triage is challenging because the impacts of a network breach can be far-reaching with unpredictable consequences. This highlights the importance of automating this process. In this paper we propose AutoCRAT, a system for quantifying the breadth and severity of threats posed by a network exposure, and for prioritizing cyber triage activities during incident response. Specifically, AutoCRAT automatically reconstructs what we call alert trees, which track network security events emanating from, or leading to, a particular computer on the network. We validate the usefulness of AutoCRAT using a real-world dataset. Experimental results show that our prototype system can reconstruct alert trees efficiently and can facilitate data visualization in both incident response and threat intelligence analysis.

==> old-threat-model.tex <==
The threat model for APIN consists of the following attacks:

\begin{enumerate}
    \item Target Diversion. An attacker may conduct attacks against a secondary target in order to distract defenders so that attacks against the primary target go unnoticed by the defender, or are pushed to a lower priority. 
    \item IDS Evasion. An attacker may use a variety of techniques to make their attacks go unnoticed. This includes any IDS evasion techniques, since much of APIN depends on the IDS output. In the host-based APIN model, attackers must also use evasion techniques that do not utilize the login function of the operating system. This means they cannot use SMB file sharing to upload malware, which might evade an IDS but would not evade the security log.
    \item Flooding. An attacker may attempt to make the runtime of APIN prohibitive by increasing the connectedness of nodes within their control. As discussed with respect to routers, this attack can significantly impact the algorithm's runtime. A na\"ive solution to this attack is to blacklist the flooded node, but this may lead to an obfuscation attack.
    \item Obfuscation. Under flooding (which may induce node blacklisting) or evasion, a link may be removed from a path. This causes one or more nodes to be separated from the path, reducing its CTS. In the case of evasion, this attack fails if even a single event follows the obfuscated link.
    \item Origin Diversion. An attacker may use two distinct nodes to conduct attacks against a single target, where each attacker node performs a different function (e.g., a scan and an exploit). In this attack, the attacker hopes to misdirect APIN so that it ranks the scanning path higher than the exploiting path. If this is achieved, the defender may falsely believe that the target was not truly attacked and therefore not compromised, even though it may have been (by the secondary attacker node).
    \item Window Flushing. An attacker may attempt to evade APIN by waiting long periods of time between attacks, in order to exploit storage or runtime limitations in the model. For example, the defender might choose to store only 30 days of traffic in their APIN database, adding new alerts as they come and flushing older ones. In this case, the attacker could evade APIN by waiting 31 days between attacks, disrupting the association of links within the reconstructed paths.
\end{enumerate}

{\color{green}
Based on these threats, we must make the following assumptions in order to ensure the robustness of APIN:
\begin{enumerate}
    \item Accuracy of the NIDS. In the ideal case, quality input in attack events should lead to quality output. When this assumption is broken, the attack path structure may lose its meaning or actively hinder network monitoring efforts. This assumption may be problematic in practice, because it is often the case that binary classifiers (e.g., anomaly detectors) have higher accuracy than categorical classifiers (i.e., IDSs which utilize the $\SID$ feature).
\end{enumerate}
}

==> related-work.tex <==

%This paper is an extension of our previous work, \cite{apin}, which introduced the concept of a threat score, and used it to rank computers and attack paths within a network. This fits into the broader category of alert prioritization.



==> results.tex <==
\subsection{Configuration}
Because the attack paths are derived from the output of an existing IDS (in this case, Suricata 4.0 \cite{suricata}), it is important that the IDS is properly configured for the network in question. For our experiments, we keep the configuration changes minimal, keeping in mind that our hope is that APIN will be useful to analysts even without advanced expertise and that many enterprise networks already incorporate their own custom configurations. Specifically, we ensure that the $home\_net$ variable is specified according to the architecture given in the datasets, and we download the most updated version of the well-reputed Emerging Threats ruleset \cite{emerging_threats_2019}, with the exception of the policy-based rules, which we exclude because the datasets do not specify what software use policies were implemented during the data collection. 

The experiments were processed using an Intel Xeon X5650 (2.67GHz) CPU running ESXi 6.5.0, with two allocated VMS, one for the APIN driver and one for the database. The driver was allocated 2 cores, 32 GB RAM, and 48 GB HDD and ran Ubuntu 18.04.3 LTS Desktop. The database was allocated 4 cores, 16 GB RAM, and 100GB HDD and ran Ubuntu 16.04.2 LTS Server. They were attached to the same virtual subnet.

\subsection{DARPA99 results}
The 16,616 alerts from Suricata's output for DARPA99 were converted from text to JSON format in 1.06s. The graph of 431 nodes was constructed and indexed in 8.70s. APIN completed in 0.67s. We consider this runtime to be satisfactory.

Because of the architecture used to collect the DARPA99 data, the results produced by APIN were severely limited. First, the simplicity of many of the attacks limits our ability to identify multi-step attacks because those used in the experiment seem to consist exclusively of a single link, where the attacker stopped the attack once the target was compromised and began a new attack, rather than pivoting between multiple internal nodes. Specifically, all of the paths identified by APIN contained one node in the ``172.16.112.0/20'' subnet and one node from another subnet or network. In this case, APIN is not useful. Nevertheless, understanding this limitation allows us to draw the following insight.
\begin{insight}
Research datasets designed to model network attacks should include multi-step attacks.
\end{insight}
%It may be worth distinguishing whether multi-step attacks belong in datasets designed to model general attacks, APTs, or some other specific threat model, but we leave this to future work.

\subsection{CSECICIDS2018 results}
According to the data description provided by its authors, the CSECICIDS2018 dataset contains a network of 450 benign nodes and a separate network of 50 attacker nodes \cite{sharafaldin2018toward}. During processing, we observed an unusually high connectedness for a network of this size. Specifically, we identified 406 nodes that had over 1000 inbound neighbors (i.e., those which produced alerts when processed by Suricata) over the span of data collection, with the highest reaching 5992. This phenomenon seems to be the result of either mass spoofing by the attacker network (which is not clearly detailed in the data description) or of some third-party interference during the experiment. In this particular case, we found that 11 of the 14 documented victims were in the top 406 highly-connected nodes.
This complexity prevents the real-time parsing of the graph, which grows exponentially. Nevertheless, we draw some insight from this limitation:
\begin{insight}
High-granularity network segmentation is important for the efficient analysis of attack paths. 
\end{insight}

Following this observation, we chose to blacklist the nodes with over 1000 inbound neighbors, preferring a partial result over a prohibitive runtime. 

The 3,323,426 alerts from Suricata's output for CSECICIDS2018 were converted from text to JSON format in 3m10s. The graph of 97,873 nodes was constructed and indexed in 29m16s. APIN completed in 42.08s. Given that alert processing and graph construction can proceed during data collection (which spanned a week), we consider this runtime to be satisfactory for the size of the dataset.

Another phenomenon in the APIN output is the frequent occurrence of attempts to probe or exploit the vulnerability known as EternalBlue (MS17-010). This observation was noted for 4 of the top 5 paths and many besides, and was triggered by several different Emerging Threats signatures: [1:2025649:2], [1:2025992:1], [1:2025650:2]. Because the publishers of the dataset do not describe any attacks using EternalBlue or otherwise targeting SMB (the protocol which EternalBlue targets), this supports our previous suspicion that some of the traffic in the dataset was produced by external sources. If this is the case, it may have implications for the validity of ground truth for other experiments (such as training machine-learning based IDSs). From this, we draw the following insight:
\begin{insight}
Datasets collected from networks with internet access should have strict controls over gateway traffic, on par with those used in production networks.
\end{insight}

The highest-ranked path (with a CTS of 34.31) contains five nodes (A-E) across four links. Its detail are below. Alert descriptions have been modified to improved readability, and SIDs have been included for reference. External IP Addresses have been truncated to preserve anonymity.
\begin{enumerate}
    \item 103.aaa.aaa.aaa (A) to 172.31.67.46 (B)
    \begin{itemize}
        \item (1:2102465:9) SMB share access
		\item (1:2102466:9) SMB unicode share access
		\item (1:2025649:2) ETERNALBLUE Probe MS17-010 (MSF style)
		\item (1:2025992:1) ETERNALBLUE Probe MS17-010 (Generic Flags)
    \end{itemize}
	\item 172.31.67.46 (B) to 103.ccc.ccc.ccc (C)
    \begin{itemize}
		\item (1:2025650:2) ETERNALBLUE Probe Vulnerable System Response MS17-010
    \end{itemize}
	\item 103.ccc.ccc.ccc (C) to 172.31.66.112 (D)
    \begin{itemize}
		\item (1:2102466:9) SMB unicode share access
		\item (1:2102465:9) SMB share access
		\item (1:2025649:2) ETERNALBLUE Probe MS17-010 (MSF style)
		\item (1:2025992:1) ETERNALBLUE Probe MS17-010 (Generic Flags)
    \end{itemize}
	\item 172.31.66.112 (D) to 54.eee.eee.eee (E)
    \begin{itemize}
		\item (1:2016149:2) Session Traversal Utilities for NAT (STUN Binding Request)
    \end{itemize}
\end{enumerate}

We can clearly see that the attacker probes node B in link 1, which is verified as vulnerable in link 2. This sequence may be indicative of a reflected attack (in which the response calls back to an IP distinct from the one used to initiate the attack), of a two-part attack (in which the attacker probes from node A and launches the full exploit from node C), or of two probes from distinct attackers. The precise meaning of this interaction is not clearly discernible by APIN because of the nature of the model. Specifically, because the model is directional and acyclical, APIN only describes one side of each connection. In any case, this can be manually verified now that APIN has ranked its threat score appropriately. 
Note that the output given above does not show the temporal relationship between alerts, except in that at least one alert of a given link must precede at least one alert of all following links. 

==> threat-score.tex <==
%Specifically, APIN selects the nodes with the highest Independent Threat Score (ITS, which is defined in Section \ref{threat-score}), and conducts queries using each as a potential victim or origin. 
%This is discussed in more detail in Section \ref{threat-score}.
%Threat score is an existing concept which has yet to be standardized. 
\ignore{
Intuitively, threat score measures the volume, cost and complexity of attacks against a node or group of nodes. Our approach is to calculate the Independent Threat Score (ITS) for each node on its own, then for each path, to aggregate the threat against all computers in the path into a Composite Threat Score (CTS), which are defined below. 

{\color{red}
In what follows we define two notions.

\begin{definition}[Independent Threat Score (ITS)]

\end{definition}

... better give an example to help understand the idea ...

\begin{definition}[Composite Threat Score (CTS)]

\end{definition}

... better give an example to help understand the idea ...

}

{\color{red}Note that ITS is defined with respect to a suspected target or origin node???.
When a defender is unable to identify a suspected target or origin node,} APIN can automatically select some of the nodes with the highest ITS and query each of them using both the target-centered and the origin-centered algorithms. This means that it may be necessary to calculate ITS before identifying paths {\color{red}(contrary to the logical structure of APIN shown in Fig. \ref{fig:framework-top-level}). This does not affect the efficiency or effectiveness of APIN.}\footnote{confusing} 
}

\ignore{
\begin{enumerate}
    \item {\bf Independent Threat Score (ITS).} The first computation considers the events incoming, within, and outgoing with respect to a particular system. This stage is repeated for each system in the network and we predict the ITS based on the relevant events. 
    %\item {\bf Dependent Threat Score (DTS).} The second stage adjusts each system's probability of compromise based on those adjacent to it in a potential attack path. This stage is designed to improve accuracy in the event of missing data, such as the use of 0-day attacks, advanced evasion techniques or manipulated log files. 
    \item {\bf Composite Threat Score (CTS).} The final computation considers the DTS of every system in an attack path and calculates the relative threat posed by the attack path as a whole. 
\end{enumerate}
The threat scores given by this method are meant to be relative indicators of the volume and severity of malicious activity along the path. They should be used to prioritize incident response efforts when compared with other scores which were calculated in the same way. Threat score should not be considered a standardized metric, as this is an open research problem. 
}


\ignore{
\subsubsection{Dependent Threat Score}

Given a potential attack path and the ITS for each computer in the path, the DTS of a single computer in the path (the {\em reference node}) is calculated using the ITS of the reference node and each of the nodes adjacent to it in the attack path. For linear paths this is exactly 3 ITS values, but for cyclical paths may include arbitrarily many, depending on the complexity of cycles allowed in the graph.

For example, if a node in an attack path is sandwiched between two nodes with much higher ITS, it is likely that some events were missed and the DTS should be higher than the same node's ITS. 

The design for DTS calculation is guided by the following principles: 
\begin{itemize}
    \item A node's DTS should not be lower than its ITS. This follows the intuition that false-negative alerts are more dangerous than false-positives. Specifically, missing an attack imposes risk to the network, whereas the misclassification of benign traffic merely imposes a delay in network analysis.
    %\item A node's DTS might be higher than the ITS of itself or any of its neighbors. Readers may find this counter-intuitive because it is natural to assume that two attacks against different computers are independent. However, because of the causality implied by the attack path structure, the observation of multiple attacks in such a chain might lead to a greater threat than any one of the attacks on its own.
    \item The number of neighbors for a node in the path should not change the range of values in the DTS output. This principle is designed to prevent the ballooning of threat score values for cyclical paths. One consequence of this principle is that DTS must not be the product or sum of the available ITSs.
    \item The nodes at either end of the path should not having diminished values because they only have a single neighbor each. 
    \item Replacing a single node with a node of lower ITS should cause the new node to also have a lower DTS within the path. This follows the intuition that a node with much malicious activity is more likely to be in a given attack path than one with very little malicious activity.
\end{itemize}

Based on these principles, we use the following formula to define DTS in our model:
\begin{equation}
    DTS(x) = \sqrt[5]{ITS(x) \cdot ITS(x.pred)^2 \cdot ITS(x.succ)^2}
\end{equation}
}


We introduce the concept of CTS to quantify the threat posed against a given path as a whole. The purpose of this definition is to gain insight into the attacker's intent and/or objective. In part, this can be inferred based on the amount of resources directed at individual computers in a path (given by the ITS). Additionally, the length of a path may be a partial indicator of how well-defined the attacker's objective may be (e.g., if their first target is their only target, perhaps the attacker has some inside knowledge about the location of data they seek to compromise). Based on these principles, we define CTS as follows:
\begin{definition}[CTS]
    The CTS of an attack path is the sum of the ITS of all nodes in the given attack path.
\end{definition}

%\subsubsection{Composite Threat Score}
%The composite threat score is calculated as the sum of the ITS of the nodes within the path.
Threat score is conceptualized independently of path identification in Figure \ref{fig:threat-score}. Specifically, this figure highlights the fact that even though ITS may be calculated for each node individually, CTS requires both the path structure and the ITS of each node in that path.

The CTS calculation is designed to rank the paths containing those computers most targeted by an attacker, even if not all attacks incident to nodes in that path follow the path precisely. For example, an attacker may conduct some attacks from a variety of external nodes (e.g., using spoofing or a botnet). In this case, it is more important to model the threat against the target than to precisely determine which attacker realized the compromise of that node. Because of this, the measurement of ITS for nodes in a path may be impacted by attacks from/to computers not in the path.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\linewidth]{figures/APIN-framework.pdf}
    \caption{Threat Score Calculation}
    \label{fig:threat-score}
\end{figure}
